Analysis of Male and Female Speakers' Word Choices in Public Speeches

The extent to which men and women use language differently has been questioned previously. Finding clear and consistent gender differences in language is not conclusive in general, and the research is heavily influenced by the context and method employed to identify the difference. In addition, the majority of the research was conducted in written form, and the sample was collected in writing. Therefore, we compared the word choices of male and female presenters in public addresses such as TED lectures. The frequency of numerous types of words, such as parts of speech (POS), linguistic, psychological, and cognitive terms were analyzed statistically to determine how male and female speakers use words differently. Based on our data, we determined that male speakers use specific types of linguistic, psychological, cognitive, and social words in considerably greater frequency than female speakers.

==> tables/liwc-example.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\onecolumn
\label{tab:liwc-example}
\bottomcaption{The mean and standard deviation of the word count in male and female transcripts across 43 LIWC categories. Additionally, examples of words from each category are provided. There was no statistically significant difference in mean between male and female speakers in the highlighted categories.}

\tablehead
{\toprule
\multicolumn{1}{c}{}                           & \multicolumn{1}{c}{}                          & \multicolumn{2}{c}{Mean}                              & \multicolumn{2}{c}{SD}                                \\
\multicolumn{1}{c}{\multirow{-2}{*}{Category}} & \multicolumn{1}{c}{\multirow{-2}{*}{Example}} & \multicolumn{1}{c}{male} & \multicolumn{1}{c}{female} & \multicolumn{1}{c}{male} & \multicolumn{1}{c}{female} \\
\midrule}
\begin{center}
\begin{supertabular*}{\linewidth}{llllll}
\multicolumn{6}{l}{\textbf{Linguistic Dimension}}                                                                                                                                                              \\
\midrule
Function                                       & whence;we                                     & 1,391.372                & 1,206.161                  & 577.947                  & 520.842                    \\
Pronoun                                        & it;you                                        & 333.667                  & 289.195                    & 149.261                  & 137.729                    \\
\rowcolor[HTML]{9AFF99} 
Personal Pronoun                               & them;thoust                                   & 155.278                  & 144.114                    & 74.642                   & 74.268                     \\
\rowcolor[HTML]{9AFF99} 
1st Person Plural Pronoun                      & ourselves;let's                               & 48.229                   & 42.460                     & 33.427                   & 30.927                     \\
2nd Person Pronoun                             & you'll;ye                                     & 46.482                   & 33.899                     & 32.573                   & 27.819                     \\
Impersonal pronouns                            & who's;anything                                & 178.171                  & 144.903                    & 85.001                   & 74.170                     \\
Article                                        & the;an;a                                      & 183.625                  & 148.503                    & 80.111                   & 62.264                     \\
Preposition                                    & after;respecting                              & 319.034                  & 282.356                    & 131.641                  & 118.568                    \\
Auxiliary verb                                 & thats;it'd                                    & 199.135                  & 171.299                    & 86.718                   & 81.003                     \\
Adverb                                         & ever;especially                               & 140.802                  & 120.990                    & 65.720                   & 61.395                     \\
\rowcolor[HTML]{9AFF99} 
Conjunction                                    & when;howre                                    & 171.439                  & 155.970                    & 75.201                   & 70.053                     \\
\rowcolor[HTML]{9AFF99} 
Negation                                       & don't;shan't                                  & 40.003                   & 35.450                     & 21.833                   & 20.218                     \\
\midrule
\multicolumn{6}{l}{\textbf{Other Grammar}}                                                                                                                                                                     \\
\midrule
Verb                                           & managed;surfs                                 & 1,856.532                & 1,612.326                  & 908.031                  & 818.422                    \\
Adjective                                      & equal;scariest                                & 94.953                   & 83.849                     & 41.491                   & 39.073                     \\
Comparison                                     & fattiest;healthier                            & 53.070                   & 47.195                     & 25.455                   & 24.738                     \\
Interrogative                                  & how's;howd                                    & 47.051                   & 41.178                     & 24.405                   & 22.582                     \\
Number                                         & four;tenth                                    & 27.804                   & 22.607                     & 16.566                   & 12.710                     \\
Quantifier                                     & sampl;each                                    & 55.467                   & 47.396                     & 27.354                   & 24.738                     \\
\midrule
\multicolumn{6}{l}{\textbf{Psychological Processes}}                                                                                                                                                           \\
\midrule
Affective Process                              & friendliest;gentler                           & 731.543                  & 643.785                    & 372.199                  & 354.008                    \\
Positive emotion                               & fearless;(                                    & 695.762                  & 614.268                    & 352.810                  & 342.799                    \\
Social processes                               & talking;excus                                 & 1,136.462                & 924.963                    & 651.324                  & 538.136                    \\
Cognitive processes                            & couldnt;need'nt                               & 660.476                  & 568.500                    & 316.392                  & 282.146                    \\
\rowcolor[HTML]{9AFF99} 
Insight                                        & wiser;knowledg                                & 48.602                   & 43.896                     & 28.269                   & 25.597                     \\
Causation                                      & comply;provok                                 & 39.515                   & 34.919                     & 19.743                   & 18.150                     \\
Discrepancy                                    & needs;could've                                & 33.684                   & 29.047                     & 18.622                   & 17.041                     \\
Tentative                                      & nearly;disorient                              & 121.143                  & 101.765                    & 57.549                   & 48.100                     \\
Certainty                                      & factual;accura                                & 30.834                   & 26.742                     & 16.213                   & 15.116                     \\
Differentiation                                & nor;respective                                & 90.079                   & 79.409                     & 43.286                   & 41.288                     \\
Perceptual processes                           & bittersweet;butter                            & 48.846                   & 42.232                     & 26.355                   & 25.144                     \\
See                                            & shine;selfie                                  & 26.406                   & 21.792                     & 17.289                   & 16.141                     \\
Drives                                         & associations;orders                           & 408.641                  & 333.020                    & 212.684                  & 174.013                    \\
Affiliation                                    & socially;confiding                            & 92.258                   & 81.826                     & 48.664                   & 44.677                     \\
Achievement                                    & obtain;attain                                 & 27.246                   & 23.715                     & 15.116                   & 13.994                     \\
Power                                          & parliament;ambitions                          & 138.243                  & 110.705                    & 74.478                   & 60.190                     \\
Reward                                         & add;takes                                     & 26.496                   & 21.956                     & 15.985                   & 14.337                     \\
\rowcolor[HTML]{9AFF99} 
Past Focus                                     & appeared;sung                                 & 149.793                  & 139.685                    & 89.218                   & 80.806                     \\
Present Focus                                  & believe;cashes                                & 861.383                  & 736.258                    & 416.913                  & 371.871                    \\
Future Focus                                   & i'mma;expect                                  & 26.156                   & 20.537                     & 16.197                   & 13.496                     \\
Relativity                                     & young;slowing                                 & 301.238                  & 255.114                    & 130.221                  & 113.037                    \\
Motion                                         & catch;lunge                                   & 45.904                   & 37.460                     & 24.249                   & 20.790                     \\
Space                                          & biggest;lil                                   & 167.501                  & 139.688                    & 77.001                   & 65.491                     \\
Time                                           & presently;modernly                            & 92.210                   & 80.913                     & 42.411                   & 37.788                     \\
\rowcolor[HTML]{9AFF99} 
Work                                           & hiring;legals                                 & 31.227                   & 28.409                     & 21.539                   & 19.167 \\
\bottomrule
\end{supertabular*}
\end{center}
\twocolumn
% }


==> tables/liwc-welch.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\begin{tabular}{lllllllll}
             & \multicolumn{2}{c}{Mean} & \multicolumn{2}{c}{SD} & \multirow{2}{*}{p} & \multirow{2}{*}{statistic} & \multirow{2}{*}{DFd} & \multirow{2}{*}{significance} \\
Category     & Female      & Male       & Female     & Male      &                    &                            &                      &                               \\
Achieve      & 26.128      & 26.128     & 14.854     & 14.854    & 0.000              & 12.310                     & 621.051              &                               \\
Adjective          & 91.437      & 91.437     & 41.046     & 41.046    & 0.000              & 15.810                     & 611.291              &                               \\
Adverb       & 134.528     & 134.528    & 65.007     & 65.007    & 0.000              & 20.270                     & 615.860              &                               \\
Affect       & 703.751     & 703.751    & 368.618    & 368.618   & 0.001              & 12.110                     & 605.716              &                               \\
Affliation   & 88.954      & 88.954     & 47.662     & 47.662    & 0.001              & 10.480                     & 625.868              &                               \\
Article      & 172.503     & 172.503    & 76.651     & 76.651    & 0.000              & 53.650                     & 729.026              &                               \\
Auxiliary verb      & 190.320     & 190.320    & 85.890     & 85.890    & 0.000              & 22.980                     & 615.915              &                               \\
Cause        & 38.060      & 38.060     & 19.362     & 19.362    & 0.000              & 12.340                     & 625.104              &                               \\
Certain      & 29.538      & 29.538     & 15.980     & 15.980    & 0.000              & 14.240                     & 616.976              &                               \\
Cognitive process      & 631.349     & 631.349    & 308.794    & 308.794   & 0.000              & 20.010                     & 643.015              &                               \\
Compare      & 51.209      & 51.209     & 25.365     & 25.365    & 0.001              & 11.280                     & 593.835              &                               \\
conjunction  & 166.540     & 166.540    & 73.924     & 73.924    & 0.002              & 9.470                      & 617.474              & Not Significant               \\
DIffer       & 86.700      & 86.700     & 42.930     & 42.930    & 0.000              & 13.190                     & 604.120              &                               \\
Discrepancy      & 32.216      & 32.216     & 18.255     & 18.255    & 0.000              & 14.210                     & 627.762              &                               \\
Drivers      & 384.693     & 384.693    & 204.206    & 204.206   & 0.000              & 33.250                     & 696.218              &                               \\
Past Tense     & 146.592     & 146.592    & 86.727     & 86.727    & 0.085              & 2.980                      & 633.799              & Not Significant               \\
Future Tense  & 24.376      & 24.376     & 15.606     & 15.606    & 0.000              & 30.980                     & 684.698              &                               \\
Present Tense & 821.758     & 821.758    & 407.182    & 407.182   & 0.000              & 21.320                     & 642.880              &                               \\
Function     & 1,332.718   & 1,332.718  & 566.810    & 566.810   & 0.000              & 23.990                     & 636.756              &                               \\
insight      & 47.112      & 47.112     & 27.525     & 27.525    & 0.011              & 6.430                      & 633.968              & Not Significant               \\
Interrog     & 45.191      & 45.191     & 23.987     & 23.987    & 0.000              & 13.080                     & 621.341              &                               \\
I pronoun        & 167.635     & 167.635    & 83.141     & 83.141    & 0.000              & 37.270                     & 656.138              &                               \\
Motion       & 43.230      & 43.230     & 23.529     & 23.529    & 0.000              & 30.150                     & 666.932              &                               \\
negate       & 38.561      & 38.561     & 21.429     & 21.429    & 0.002              & 9.810                      & 620.870              & Not Significant               \\
Number       & 26.158      & 26.158     & 15.631     & 15.631    & 0.000              & 27.870                     & 737.367              &                               \\
Percept      & 46.751      & 46.751     & 26.146     & 26.146    & 0.000              & 13.660                     & 603.996              &                               \\
Positive Emotion       & 669.954     & 669.954    & 351.541    & 351.541   & 0.001              & 11.300                     & 593.961              &                               \\
Power        & 129.522     & 129.522    & 71.396     & 71.396    & 0.000              & 36.490                     & 704.045              &                               \\
Personal Pronoun        & 151.743     & 151.743    & 74.666     & 74.666    & 0.033              & 4.590                      & 581.232              & Not Significant               \\
Prepositions         & 307.419     & 307.419    & 128.720    & 128.720   & 0.000              & 18.150                     & 637.086              &                               \\
Pronoun      & 319.583     & 319.583    & 147.098    & 147.098   & 0.000              & 20.120                     & 622.935              &                               \\
Quant        & 52.911      & 52.911     & 26.805     & 26.805    & 0.000              & 20.240                     & 634.675              &                               \\
Relative     & 286.631     & 286.631    & 126.806    & 126.806   & 0.000              & 30.720                     & 659.321              &                               \\
Reward       & 25.058      & 25.058     & 15.618     & 15.618    & 0.000              & 18.960                     & 639.588              &                               \\
See          & 24.945      & 24.945     & 17.061     & 17.061    & 0.000              & 15.900                     & 616.219              &                               \\
Social       & 1,069.484   & 1,069.484  & 625.239    & 625.239   & 0.000              & 27.420                     & 690.033              &                               \\
Space        & 158.693     & 158.693    & 74.648     & 74.648    & 0.000              & 32.760                     & 671.883              &                               \\
Tentative       & 115.006     & 115.006    & 55.446     & 55.446    & 0.000              & 29.080                     & 682.764              &                               \\
Time         & 88.632      & 88.632     & 41.319     & 41.319    & 0.000              & 16.820                     & 643.535              &                               \\
verb         & 1,779.196   & 1,779.196  & 887.514    & 887.514   & 0.000              & 16.890                     & 636.676              &                               \\
we           & 46.402      & 46.402     & 32.750     & 32.750    & 0.010              & 6.730                      & 621.391              & Not Significant               \\
Work         & 30.335      & 30.335     & 20.848     & 20.848    & 0.044              & 4.060                      & 644.296              & Not Significant               \\
you          & 42.497      & 42.497     & 31.677     & 31.677    & 0.000              & 37.280                     & 669.313              &                              
\end{tabular}
\caption{Univariate Welch Anova Test}
\label{tab:liwc-welch}
\end{table*}
